ARIDA - Active railway infrastructure dataset annotation using neural network predictions

Modern railway perception requires large comprehensive image datasets, but creating them is slowed by manual labeling, especially for track polylines and other complex infrastructure geometry. This paper presents the Active Railway Infrastructure Dataset Annotation framework, a railway-specific semi-automated pipeline that converts instance predictions from a mask scoring instance segmentation network into bounding-boxes, polygons, polylines, and paired polylines. To keep automatic track geometry annotation reliable without ground truth, it applies confidence thresholds and an unique contour-agreement quality score as an acceptance gate. An active learning loop ranks remaining images by uncertainty and adapts the number of manual queries per cycle. This is achieved through a novel quantity control mechanism, in which easy images are auto-accepted and human effort targets hard cases. Experiments on disjoint, diverse imagery and time-sequential, redundant imagery quantify effort reduction and accuracy trade-offs, achieving about two thirds reduction in the disjoint regime and up to 93% in the sequential regime. The study also provides guidance for initial label budgets and stopping to avoid over-annotation.

==> Settings/Debug_Markers.tex <==
% % Kennzeichnungsbefehle
%     % Anmerkungen kennzeichnen
%         \definecolor{annotation}{RGB}{0, 192, 223}
%         \newcommand{\annot}[1]{\textcolor{annotation}{\textsc{\#T:}} \textbf{#1}}

%         % \newcommand{\annot}[1]{}

%     % Anmerkung bearbeitet
%         \definecolor{annotationdone}{RGB}{0, 192, 0}
%         \newcommand{\annotdone}[1]{\textcolor{annotationdone}{\textsc{\#TD:}} \textbf{#1}}

%         % \newcommand{\annotdone}[1]{}
        
%     % Fehlendes Zitat
%         \definecolor{citneeded}{RGB}{255, 0, 127}
%         \newcommand{\citneeded}[1]{\textcolor{citneeded}{\textsc{\#ZF:}} \textbf{#1}}      

%         % \newcommand{\citneeded}[1]{} 

%     % Fehlende Referenz
%         \definecolor{refneeded}{RGB}{255, 0, 127}
%         \newcommand{\refneeded}[1]{\textcolor{refneeded}{\textsc{\#RF:}} \textbf{#1}}

%         % \newcommand{\refneeded}[1]{}

%     % Fehlende Grafik
%         \definecolor{graphicsneeded}{RGB}{255, 0, 127}
%         \newcommand{\graphicsneeded}[1]{\textcolor{graphicsneeded}{\textsc{\#GRF:}} \textbf{#1}}

%         % \newcommand{\graphicsneeded}[1]{}            

%     % Debug Markierung
%         \definecolor{dbg1}{RGB}{255, 127, 0}
%         \newcommand{\dbg}[1]{\textcolor{dbg1}{\textsc{\#D:}} \textbf{#1}}

%         % \newcommand{\dbg}[1]{}
    
%     % Bin-mir-unsicher-Markierung
%         \definecolor{notsure}{RGB}{255, 64, 0}
%         \newcommand{\notsure}[1]{\textcolor{notsure}{\textsc{\#?:} \textit{#1}}}

%         % \newcommand{\notsure}[1]{}
